The State of the Art in Creating Visualization Corpora for Automated Chart Analysis

We present a state-of-the-art report on visualization corpora in automated chart analysis research. We survey 56 papers that created or used a visualization corpus as the input of their research techniques or systems. Based on a multi-level task taxonomy that identifies the goal, method, and outputs of automated chart analysis, we examine the property space of existing chart corpora along five dimensions: format, scope, collection method, annotations, and diversity. Through the survey, we summarize common patterns and practices of creating chart corpora, identify research gaps and opportunities, and discuss the desired properties of future benchmark corpora and the required tools to create them.

==> sections/Proposed_Structure.tex <==
\section{Survey Method and Proposed Structure}
We will start with the recent survey on artificial intelligence approaches for data visualization~\cite{wu2021ai4vis}, which consists of 98 publications from 10 research areas,
% that are related to general AI approaches for data visualization, and collected 
and identify papers that explicitly introduced a visualization corpus as the input of their techniques or systems. 
% We exclude works that involve other kinds of inputs, e.g., chart-based QA systems~\cite{kahou2017figureqa,kahou2017figureqa,singh2020stl} where NLP techniques are employed to parse text-based questions. 
Our preliminary paper collection contains 40 publications and will continue to grow.

The survey will be structured based on two main orthogonal dimensions: corpus properties, and multi-level task abstractions. We will characterize the features of existing visualization corpora, and examine how well these corpora provide a basis for supporting and evaluating the outcomes of the chart analysis and repurposing tasks. 
% Through the survey, we hope to summarize common practices and pitfalls in the current chart understanding methods and applications, formulate guidelines for creating visualization corpora to promote reproducible and verifiable scientific progress, and identify research gaps and opportunities. The plan is to make our taxonomies and analysis public as an interactive web-based collection~\cite{beck2015visual}.

% The primary structure of this survey is based on the set of dimensions of visualization corpora we extracted from related papers. In addition, we will build a taxonomy of tasks that are performed at the chart level, and use this categorization to thoroughly analyze how the dimensions of corpora are decided and formed. Our goal is not only to provide a comprehensive overview of properties of visualization corpora, but also to examine how well these tasks are supported by the corpora, identify the common practices~(and potential misunderstandings) in the current literature, and formulate a complete and scalable guideline for creating visualization corpora. The plan is to make our categorization and analysis public online as an interactive web-based collection~\cite{beck2015visual}.
\vspace{-0.35cm}

\subsection{Corpus Properties}
A primary contribution of this survey will be an analysis of the properties of visualization corpora. The following list contains some properties we plan to include in our analysis.

% We will extract the dimensions list below from corpora used in the surveyed papers, while it is possible that we include more dimensions that will benefit our analysis in the final version.

\bpstart{Format} refers to the file type of visualizations in a corpus, which includes bitmap graphics~(.jpeg, .png)~\cite{savva2011revision,tang2016deepchart,jung2017chartsense,poco2017reverse,poco2017extracting,deng2022visimages}, vector graphics~(.svg)~\cite{harper2014deconstructing,harper2017converting,battle2018beagle,wu2020mobilevisfixer,li2022structure}, and programs~\cite{dibia2019data2vis,mcnutt2021integrated,zhao2020chartseer,kim2020answering}. 
% Our collection contains more bitmap corpora than vector corpora. This is possibly due to the fact that raster images are more readily available and easier to collect. However, this doesn't make the bitmap format the best option for all the visualization analysis tasks, since the vector-based format has unique advantages~(e.g., its raw text contains type and coordinate information of graphical marks). We will analyse the pros and cons of both formats in practice and compare them under different tasks.

\bpstart{Scope} refers to the assumptions or selection criteria about the visualizations in a corpus. These are usually specified to constrain the research problem space. 
% closely related to the targeted input and the limitations of their work. 
We identify two kinds of scopes: \textit{chart design} and \textit{chart source}. \textit{Chart design} can be described using high-level chart typologies, for example, \cite{prasad2007classifying} classify charts into bar charts, curve plots, pie charts, scatter plots and surface plots; \cite{kafle2018dvqa,cui2021mixed} focus on reusing bar charts. In addition to chart type, we plan to also analyze \textit{chart design} in terms of finer-grained constraints, including but not limited to: composite arrangement (e.g., \cite{chen2020composition} focuses on decomposing and understanding multiple-view visualizations), mark and glyph type (e.g., \cite{chen2019towards} retargets complex glyphs in infographics), and superimposition status (e.g.,~\cite{poco2017reverse} assumes non-composed single-layer figures). 
% We identify three kinds of scopes: (1) \textit{chart type}, for example, \cite{prasad2007classifying} classify charts into bar charts, curve plots, pie charts, scatter plots and surface plots,~\cite{dai2018chart} extracts text and numbers from bar charts, pie charts, line charts, scatter plots and radar charts, and~\cite{cui2021mixed} focuses on reusing infographic bar charts; (2) \textit{chart structure}, examples include~\cite{chen2020composition} that considers general multiple-view visualizations,~\cite{chen2019towards} that targets at info-graphics of the timeline layout, and~\cite{poco2017reverse} that assumes non-composed single-layer figures with a Cartesian coordinate space; (3)
\textit{Chart source} describes how the input visualizations were generated or where they were found. 
% \textit{chart source}, 
For example, ~\cite{harper2014deconstructing,harper2017converting,hoque2019searching} require that the visualizations are created using d3.js~\cite{bostock2011d3}; \cite{ray2015architecture,al2017machine} focus on scientific figures from scholarly documents.

\bpstart{Collection method} denotes how a corpus was collected, which is influenced by both \textit{Format} and \textit{Scope}. Two main kinds of collection methods have been observed: \textit{manual curation}~\cite{huang2007system, gao2012view,demir2012summarizing, poco2017extracting,cui2019text,choi2019visualizing,qian2020retrieve} and \textit{web crawling}~\cite{chen2015diagramflyer,battle2018beagle,hoque2019searching,hu2019vizml,li2022structure}. Only three works have reused existing corpora:~\cite{savva2011revision} sampled visualizations from~\cite{prasad2007classifying} and~\cite{huang2007system} to create the Revision corpus, which was adopted and augmented with more examples by ~\cite{jung2017chartsense}; \cite{fu2019visualization} used corpora from ~\cite{borkin2013makes,harrison2015infographic,bylinskii2017understanding}. All the other papers collected their own corpora. This shows a lack of standard benchmark corpora in visualization research, as discussed in Section~\ref{sec:1}.

% However, since the total number of reused corpora is small and these works all have collected new examples for the training purpose, we don't include reusing existing corpora as a third collecting method.

\bpstart{Annotations} are labels associated with visualizations, serving as ground truth for chart analysis tasks. The commonly observed \textit{types of annotation} include  
% collected images should be labelled/annotated to accommodate requirements from the task, and the process of which might demands much work from the developer's side. Commonly-seen annotation objectives include but are not limited to 
chart type, visual encodings, chart ranking, and the bounding boxes of chart area, legend area, and x\&y axis. Two main \textit{methods of annotating} have been observed:
\textit{in-house annotating} using a custom graphical user interface is widely adopted~\cite{poco2017reverse,poco2017extracting,battle2018beagle,deng2022visimages}, and 
\textit{crowdsourced annotating} with Amazon’s Mechanical Turk (MTurk)~\cite{saleh2015learning,bylinskii2017learning,kim2018multimodal} or a professional data annotation company~\cite{deng2022visimages} is carried out for some large corpora or certain chart evaluation tasks.
Automatic annotating is possible in rare cases, e.g., in~\cite{hoque2019searching} the annotating process was automated based on the authors' previous works~\cite{harper2014deconstructing,harper2017converting}. 

% It is worth thinking that why it is hard in general to automate chart annotation, and what are potential solutions towards annotation tools for general purposes which could save people time and money. We will investigate and discuss these questions considering other dimensions and the task categorization.

% \bpstart{Annotation Process} is another important dimension of a visualization corpus that shows how the collected images should be labelled/annotated to accommodate requirements from the task, and the process of which might demands much work from the developer's side. Commonly-seen annotation objectives include but are not limited to chart type, chart area, bounding boxes of x\&y axis and labels, bounding boxes of the legend area, data encoding, and chart ranking. Two mainstream annotating process have been observed: \textit{in-house annotating} with the help of a custom GUI is widely adopted under diverse situations~\cite{poco2017reverse,poco2017extracting,battle2018beagle,deng2022visimages}, and \textit{crowdsourcing annotating} with Amazon’s Mechanical Turk (MTurk)~\cite{saleh2015learningr,bylinskii2017learning,kim2018multimodal} or a professional data annotation company~\cite{deng2022visimages} is carried out for some large corpora or certain chart evaluation tasks. Note that automatic annotating is possible in some rare case, e.g., in~\cite{hoque2019searching} the annotating process was made automatic based on the authors' previous works~\cite{harper2014deconstructing,harper2017converting}. It is worth thinking that why it is hard in general to automate chart annotation, and what are potential solutions towards annotation tools for general purposes which could save people time and money. We will investigate and discuss these questions considering other dimensions and the task categorization.

\bpstart{Diversity} measures how much the visualizations differ from one another within a corpus. This integrative property depends on factors including \textit{Format},~\textit{Scope} and~\textit{Collection method}. For example,~\cite{deng2022visimages} observed better \textit{diversity regarding chart types} in their corpus collected from visualization publications compared to previous corpora, and~\cite{li2022structure} listed \textit{diversity regarding chart sources} as one limitation since their system was trained with SVG images crawled solely from Plotly~\cite{plotly} and may meet difficulties with visualizations created with other tools. In general, diversity is an important property which could greatly influence the scalability and robustness of developed techniques or systems, and it is under-explored in the current literature compared to other properties.

% We will study dataset diversity in detail and examine its influences on the generalizability of techniques or systems.

% zhicheng.liu: I think this is about the diversity of dataset, which depends on not only the size (number of visualizations) but also format, scope and collection method

% \bpstart{Size}\chen{if space is not allowed we probably can exclude this one} measures the bigness of a corpus, which is influenced by many factors including \textit{format}, \textit{scope}, \textit{collecting method} and the task purpose. To be specific, corpus format and scope typically will narrow down the number of available image candidates~\cite{poco2017reverse}; collecting methods matters a lot since manually collected corpora usually are of a relatively small size~(Revision corpus~\cite{savva2011revision} contains 2084 examples) while crawled corpora are usually large~(FigureSeer corpus~\cite{siegel2016figureseer} contains over 60000 figures); and deep-learning-based methods~\cite{saleh2015learning, tang2016deepchart,al2017machine,hu2019vizml} usually require much larger corpora then other methods~\cite{harper2017converting,poco2017extracting,cui2019text,qian2020retrieve}. We will study the trade-offs between corpus size and other factors in detail.

% \bpstart{(6) Model}
\vspace{-0.3cm}

\subsection{Task Taxonomy}
After identifying the corpus properties, we will assess the adequacy of existing corpora in terms of how their properties support different chart analysis tasks. We plan to use a multi-level task taxonomy with the following preliminary form: 
% As we mentioned above, we will analyze corpus dimensions considering the specific tasks. 
% Here we present a preliminary chart-level taxonomy summarized from surveyed papers with representative references. \chen{I previously sketched that section 2 would be talking about multi-level tasks for most parts and discussing corpus dimensions at last for maybe not too long; while during writing I realized that focusing on corpus and put the task taxonomy as an assistant for the analysis looks more reasonable and potential is better for us to differentiate our work. Thus, I didn't detail the task part.}

\bpstart{Why: the purpose.} This task level describes the goals and applications of analyzing charts, which include and are not limited to: \textit{redesign} an existing chart \cite{savva2011revision,harper2014deconstructing}, \textit{reuse} an existing chart as templates for new data \cite{harper2017converting,chen2019towards,cui2021mixed},  \textit{retrieve} charts matching certain criteria \cite{chen2015diagramflyer,hoque2019searching,li2022structure}, and \textit{reason} about communicative information present in charts~\cite{kahou2017figureqa,chaudhry2020leaf,obeid2020chart}.

\bpstart{How: the method.} This task level describes the analysis techniques. Oftentimes multiple techniques are used in conjunction to achieve a goal. For example, to redesign an existing chart, \cite{savva2011revision,jung2017chartsense} \textit{classify} the type of chart and then \textit{extract} the underlying data; to reuse chart styles, \cite{harper2014deconstructing,harper2017converting} \textit{extract} the underlying data and then \textit{deconstruct} charts into encodings.


\bpstart{What: the components.} This task level describes the outputs of chart analysis methods, which include but are not limited to: source data~\cite{savva2011revision}, chart type~\cite{battle2018beagle}, chart quality~\cite{fu2019visualization}, similarity~\cite{saleh2015learning}, visual salience~\cite{bylinskii2017learning}, and chart components such as axis \& legend ~\cite{poco2017extracting,wu2020mobilevisfixer}, mark grouping~\cite{cui2021mixed,li2022structure}, encodings~\cite{poco2017reverse,harper2017converting}, and layouts~\cite{chen2019towards,chen2020composition}.

We will integrate this multi-level task taxonomy with the analysis of corpus properties. For example, our collection of corpora contains more bitmap corpora than vector corpora. This is possibly due to the fact that raster images are more readily available and easier to collect. However, this does not make the bitmap format the best option for all the visualization analysis and repurposing tasks, since the vector-based format has unique advantages~(e.g., its raw text contains the type and coordinate information of graphical marks). We will analyse the pros and cons of both formats in practice and compare them under different tasks.


% \bpstart{(1) Chart Type Classification} that categorizes input images into a set of chart types~\cite{prasad2007classifying,choudhury2016scalable,tang2016deepchart,battle2018beagle,deng2022visimages}. 

% \bpstart{(2) Chart Data Extraction} that either recovers the underlying \textit{tabular data}~\cite{savva2011revision,jung2017chartsense,dai2018chart} or extracts \textit{graphical data} like texts and marks~\cite{poco2017reverse,chen2019towards}.

% \bpstart{(3) Chart Semantic Comprehension} that understands semantic information that is implicitly coded within the raw contexts of an image. A more fine-grained breakdown includes \textit{axis\&legend detection}~\cite{poco2017extracting,wu2020mobilevisfixer}, \textit{mark grouping}~\cite{cui2021mixed,li2022structure}, \textit{encoding extraction}~\cite{poco2017reverse,harper2017converting}, and \textit{layout inference}~\cite{chen2019towards,chen2020composition}.

% \bpstart{(4) Chart Property Evaluation} that measures visualizations regarding certain aspects including \textit{quality}~\cite{fu2019visualization}, \textit{similarity}~\cite{saleh2015learning} and \textit{visual salience}~\cite{bylinskii2017learning}.

% Note that one work can include several tasks, e.g.~\cite{savva2011revision,jung2017chartsense} perform chart type classification before chart data extraction, and~\cite{harper2014deconstructing,harper2017converting,hoque2019searching} conduct chart data extraction first and then perform chart semantic understanding.
